Underwater Acoustic Ranging Between Smartphones

We present a novel underwater system that can perform acoustic ranging between commodity smartphones. To achieve this, we design a real-time underwater ranging protocol that computes the time-of-flight between smartphones. To address the severe underwater multipath, we present a dual-microphone optimization algorithm that can more reliably identify the direct path. Our underwater evaluations show that our system has median errors of 0.48-0.86 m at distances upto 35 m. Further, our system can operate across smartphone model pairs and works in the presence of clock drifts. While existing underwater localization research is targeted for custom hydrophone hardware, we believe that our work breaks new ground by demonstrating a path to bringing underwater ranging capabilities to billions of existing smartphones, without additional hardware.

==> eval-1.tex <==
\section{Evaluation}

\begin{figure}[t!]
    \includegraphics[width=.48\textwidth]{./figs/dist-1260}
    \vskip -0.15in
\caption{{\bf Distance}}
\vskip -0.15in
\label{fig:dist}
\end{figure}

\vskip 0.05in\noindent{\bf Range evaluation.} 
We evaluated the range of our system along a dock of a lake with a total water depth of 9~m. We performed the experiments using two Samsung Galaxy S9 phones set to transmit the preamble at the maximum speaker volume. The phones were set to transmit using the speaker at the bottom of the device, and receive using the microphones at the bottom and top of the device. We designate the two phones as being either a sender or replier. In this evaluation, the sender was configured to send a preamble to the replier every six seconds. The replier is then set to continuously run the preamble detection algorithm and respond with a preamble three seconds after it has received a preamble from the sender. We empirically select three seconds as the response time as this is the decay time of the automatic gain control on the sender's microphone. Specifically it takes the sender's microphone at least three seconds to adjust its gain to be sensitive to the environment after sending its own preamble. At each distance, the sender and replier are set to exchange preambles up to a maximum of 60 times. After 20 ranging measurements, the phones were removed from the water and submerged again.

The phones were enclosed in a waterproof pouch and attached to a selfie stick and telescopic extension pole, which was used to submerge the phones to a depth of 2.5~m. The selfie stick and extension pole were attached using waterproof tape and zip ties. This setup was chosen so that the phone's position and angle remained static during the course of a measurement. The phones were positioned so that their speakers and microphones directly faced each other.

We used a tape measure to mark different measurement distances up to a maximum of 45~m along the dock. In this evaluation we use 1500~m/s as the speed of sound underwater. We note that while the speed of sound underwater changes at large depths greater than xxx~m, the maximum depth used in all our evaluation is 8~m.

Fig.~\ref{fig:dist} shows the CDF of the distance error obtained by our system for distances up to 45~m. The plot shows that the median error of our system is is 0.86~m at 35~m, and increases to 3.27~m at 45~m. The 95th percentile error increases from 1.51~m to 3.62~m as the distance increses from 35 to 45~m. We note that in this experiments, we use a preamble with a length of 316~ms. When we use a longer preamble with a length of 479~ms, the median error of the system decreases to xxx and xxx~m at 35 and 45~m respectively. The 95th percentile of the system decreases to xxx and xxx~m and 35 and 45~m.

\begin{figure}[t!]
    \includegraphics[width=.23\textwidth]{./figs/pool}
    \includegraphics[width=.23\textwidth]{./figs/occ}
    \vskip -0.15in
\caption{{\bf Mobility}}
\vskip -0.15in
\label{fig:mobility}
\end{figure}
\vskip 0.05in\noindent{\bf Effect of mobility.} 
We measure the effect of human mobility in the challenging environment of a busy swimming pool. We performed a ranging measurement at a fixed horizontal distance of 6.1~m over a period of 8 minutes. During this time, the direct path between the sending and replying phone was frequently blocked by other swimmers. The depth of the pool was 2.5~m and the phones were held by hand at a depth of 1~m. Fig.~\ref{fig:pool} shows the CDF of the ranging error at 6.1~m. The median and 95th percentile error was 0.35 and 0.84~m respectively. 

\vskip 0.05in\noindent{\bf Effect of human occlusion.} 
We measure the effect of human occlusion from the smartphone user in the swimming pool. To do this, we would periodically block the speaker and microphone of the sending phone with our hand and body. The measurement was performed at a horizontal distance of 6.1~m over 8 minutes, and was performed when other swimmers did not block the path between the smartphones. Fig.~\ref{fig:occ} shows the CDF of the ranging error when there is human occlusion between the smartphones, and when there is no occlusion. The presence of an occlusion increased the median error from 0.31 to 0.87~m. The 95th percentile error also increased from 0.08 to 0.97~m.

\begin{figure*}[t!]
    \includegraphics[width=.19\textwidth]{./figs/motion1.pdf}
    \includegraphics[width=.19\textwidth]{./figs/motion2.pdf}
    \includegraphics[width=.19\textwidth]{./figs/motion3.pdf}
    \includegraphics[width=.19\textwidth]{./figs/motion4.pdf}
    \includegraphics[width=.19\textwidth]{./figs/motion5.pdf}
    \vskip -0.05in
\caption{Tracking}
\vskip -0.05in
\label{fig:track}
\end{figure*}
\vskip 0.05in\noindent{\bf Tracking user motion.} 
We evaluate whether our system can be used to track the 1D trajectory of the smartphone over time. In this experiment, we moved the smartphone along different 1D trajectories parallel to the coast at the dock location for measurement durations of 132 to 159~s. The smartphone was moved at speeds ranging from 6 to 14~cm/s. We obtained the ground truth distance measurement by recording a video of the smartphone's position with respect to a tape measure placed along the dock. The video recording was then synchronized with the ranging measurements obtained from the smartphones underwater. Fig.~\ref{fig:track} compares the trajectories estimated by our system with the ground truth measurements. The median and 95th percentile ranging error across all five measurements was 0.26 and 1.18~m respectively. The median error for the slowest and fastest measurement speed was 0.17 and 0.37~m respectively.

\begin{figure*}[t!]
    \includegraphics[width=.32\textwidth]{./figs/loc1}
    \includegraphics[width=.32\textwidth]{./figs/loc3}
    \includegraphics[width=.32\textwidth]{./figs/loc2}
    \vskip -0.15in
\caption{{\bf Locations (a) Dock (b) Viewpoint (c) Boathouse}}
\vskip -0.15in
\label{fig:locs}
\end{figure*}

\begin{figure}[t!]
    \includegraphics[width=.23\textwidth]{./figs/locs-gasworks}
    \includegraphics[width=.23\textwidth]{./figs/locs-greenlake}
    \vskip -0.15in
\caption{{\bf Locations}}
\vskip -0.15in
\label{fig:locs2}
\end{figure}
\vskip 0.05in\noindent{\bf Effect of different environments.} 
We evaluate our system in two additional environments: a viewpoint, and a boathouse with different water depths and noise profiles (Fig.~\ref{fig:locs}). At the viewpoint, the total water depth ranged from 1 to 1.5~m and the phones were submerged to a depth of 0.5~m. At the boathouse the total water depth of 5~m and the phones were submerged to a depth of 2.5~m. We measured the ranging error at 10, 20, and 30~m distances. Fig.~\ref{fig:locs2} shows the CDF at these locations. The figure shows that the ranging error across these distances and locations are similar with a median and 95th percentile error of 0.73 and 0.27~m at the viewpoint, and 0.72 and 0.07~m at the boathouse. The median and 95th percentile error across these distances at the dock location is 0.80 and 1.45~m.

\begin{figure}[t!]
    \includegraphics[width=.48\textwidth]{./figs/depth}
    \vskip -0.15in
\caption{{\bf Depth}}
\vskip -0.15in
\label{fig:depth}
\end{figure}
\vskip 0.05in\noindent{\bf Effect of different depths.} 
We evaluate the ranging error of our system when the smartphones are placed at different water depths at the dock location which had a total depth of 9~m. Multipath interference can be strong when the phones are positioned close to the surface or floor of the ocean, due to reflections from the top or bottom of the water body. We lowered the smartphones into the water using ropes marked at 2, 5, and 8~m. The phones were weighed down with a bag of pebbles to ensure the ropes were vertically straight. The phones were positioned at a fixed horizontal distance of 18~m. Unlike previous experiments, the rope would cause the phone to rotate and sway slowly, making it difficult to control the angle of the phone during the measurement. Fig.~\ref{fig:depth} shows the CDF of the ranging error at different depths. The figure shows that the median and 95th percentile error is lowest at 0.28 and 0.06~m at the 5~m depth, which is around the midpoint depth of the dock. In contrast, the median ranging error at 2 and 8~m are 0.33 and 0.58~m respectively. 

\begin{figure}[t!]
    \includegraphics[width=.23\textwidth]{./figs/phones}
    \includegraphics[width=.23\textwidth]{./figs/rot}
    \vskip -0.15in
\caption{{\bf Phones and rotation}}
\vskip -0.15in
\label{fig:phones_rot}
\end{figure}
\vskip 0.05in\noindent{\bf Effect of smartphone models.} 
We evaluate the effect of different smartphone model pairs on ranging error. As different smartphones use different speakers and microphones, the frequency selectivity of an acoustic signal can vary between devices. In this experiment we evaluated three different smartphones models: Samsung Galaxy S9, Google Pixel 3a, and OnePlus 8 Pro. Fig.~\ref{fig:phones_rot} shows the CDF of ranging error between different device pairs. The plot shows that the median error for a given device pair ranges from 0.28 to 0.54~m. Across all device pairs and measurements, the median and 95th percentile error is 0.41 and 0.04~m respectively.

\vskip 0.05in\noindent{\bf Effect of phone orientation.} 
We evaluate the effect of phone orientation on ranging performance at the dock at a horizontal distance of 20~m and a depth of 2.5~m. We first positioned the speaker and microphone of both phones to directly face each other so their azimuth φ and polar angle θ is set to 0° and 180° respectively. We measure the ranging error when the sender phone is rotated to different azimuth and polar angles. We first twist the pole to rotate the sender phone in the azimuth angle to 90° and 180° while keeping the polar angle constant. We then reposition the phone so it's speaker and microphone faces upwards with with φ=0°, θ=0°. Fig.~\ref{fig:phones_rot} shows the CDF of the ranging error for these different rotation configurations. The median ranging error ranges from 0.54 to 1.25~m across different orientations. The 95th percentile ranging error ranges from 0.78 to 1.62~m.

\begin{figure}[t!]
    \includegraphics[width=.4\textwidth]{./figs/compass}
    \vskip -0.15in
\caption{{\bf Compass}}
\vskip -0.15in
\label{fig:compass}
\end{figure}
\vskip 0.05in\noindent{\bf Effect of compass underwater.} 
We evaluate whether the compass bearings of a smartphone placed underwater correspond to those of a smartphone in open air. A correspondence suggests that the smartphone's compass can be used to aid in underwater navigation. In this evaluation we attached a smartphone and selfie stick to the bottom and top of the extension pole. The smartphone at the bottom end of the pole was submerged directly underwater to a depth of 3~m while the smartphone at the top end of the pole remained in air. We twisted the pole on its axis in random clockwise and anticlockwise motions and recorded the compass bearing measurements on both smartphones. Fig.~\ref{fig:compass} shows the unwrapped compass bearing angles measured by the smartphone underwater and in the air. The figure shows that the average angular error across the two measurements was 19°.

